Dynamical Regimes of Diffusion Models

Using statistical physics methods, we study generative diffusion models in the regime where the dimension of space and the number of data are large, and the score function has been trained optimally. Our analysis reveals three distinct dynamical regimes during the backward generative diffusion process. The generative dynamics, starting from pure noise, encounters first a 'speciation' transition where the gross structure of data is unraveled, through a mechanism similar to symmetry breaking in phase transitions. It is followed at later time by a 'collapse' transition where the trajectories of the dynamics become attracted to one of the memorized data points, through a mechanism which is similar to the condensation in a glass phase. For any dataset, the speciation time can be found from a spectral analysis of the correlation matrix, and the collapse time can be found from the estimation of an 'excess entropy' in the data. The dependence of the collapse time on the dimension and number of data provides a thorough characterization of the curse of dimensionality for diffusion models. Analytical solutions for simple models like high-dimensional Gaussian mixtures substantiate these findings and provide a theoretical framework, while extensions to more complex scenarios and numerical validations with real datasets confirm the theoretical predictions.

==> No_journal/natdin_et_al.tex <==
%%  natdin.bst   Vers. [3.1]  2006-01-02   mit PWD cite-multimode
%%
%%  Aenderungen seit Vers. [3.0bx]:
%%  a) Funktions-Zusaetze bei Autoren sind nun moeglich
%%  b) Internetquellen ohne Zusatz "Online--Ressource" !
%%  c) verbesserte INPROCEEDINGS, PROCEEDINGS-Funktionen
%%  d) neue TECHREPORT und MANUAL-Funktionen
%%  e) neue format.pages.book-Funktion
%%  f) neue format.online.lastchecked-Funktion
%%  
%%
%%   K.F.Lorenzen  (Copyright 1994-2006)  email:  lorenzen.marxen@t-online.de
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%  Mit diesem BibTex-style werden Literaturverzeichnisse nach dem deutschen
%%  Standard DIN 1505, Teil 2 und 3 formatiert. Die label im Quellen-/
%%  Literaturverzeichnis sind vom Typ 'Verfasser - Jahr' und
%%  entsprechen den Zitatformen im Text. Es koennen alle von
%%  Patrick W. Daly im natbib-Paket implementierten Zitierbefehle
%%  genutzt werden. Eine Kurzbeschreibung liegt als Datei natnotes.pdf zusammen
%%  mit der im Aufbau befindlichen Beschreibung des natdin-Stils
%%  unter der URL  http://www.haw-hamburg.de/pers/Lorenzen/bibtex.
%%  Eine Anleitung zur Anwendung der Norm DIN 1505 findet sich unter der
%%  URL http://www.bui.haw-hamburg.de/pers/klaus.lorenzen/ASP/litverz.pdf
%%
%%  Es werden nun auch Elektronische Online / Offline Ressourcen wie
%%  Internetquellen, CD-ROM usw. verarbeitet. Dazu kommen spezielle
%%  Publikationsformen wie Patente, Normen, Karten, Fernsehaufzeichnungen,
%%  Gesetzesstellen, Spiele u.a.
%
%%  NATDIN.BST muss zusammen mit NATBIB.STY von Patrick W. Daly und der in
%%  dieser Verteilung modifizierten Konfiguration NATBIB.CFG aufgerufen
%%  werden. NATDIN.BST ist vorzugsweise in den ...\bibtex\bst - Pfad zu
%%  stellen. Die jeweils individuelle Konfiguration NATBIB.CFG wird am
%%  besten in das Verzeichnis der LaTex-Quelle selbst gelegt.
%%
%%  Eine Muster-Konfiguration wird auf Vorschlag von Helge Baumann eingefuegt:
%   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%   NATBIB.CFG        in Verbindung mit natbib.sty     Lorenzen, 2005-05-31
%		      diese Konfigurationsdatei wird zuletzt eingelesen und
%		      enthaelt die lokal gewuenschten Einstellungen fuer den
%		      Bibliographie-- und Zitierstil
%
%   \newcommand{\bibstyle@natdin}%
%       {\bibpunct{(}{)}{;}{a}{}{,~}
%       \gdef\NAT@biblabelnum##1{\textbf{##1}\\}} %% \\ bewirkt Zeilenumbruch
%                                                 %% nach label-Ausgabe
%
%   \bibstyle@natdin
%
%   % Einzug der Belege nach der Einordnungsmarke
%   \setlength{\bibhang}{7mm}
%
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%
%%  Zur Gewaehrleistung der Allgemeingueltigkeit von bib-files gelten
%%  in den DIN-styles mit einer einzigen Ausnahme die in der Tex-Literatur
%%  veroeffentlichten originalen Definitionen und Regeln fuer die
%%  Publikationstypen (entry-types) und die bibliographischen Felder (fields).
%%  Die Ausnahme bezieht sich auf den entry-type PROCEEDINGS und das Feld
%%  address, fuer das Oren Patashnik dort die Sonderbedeutung "Konferenzort"
%%  gewaehlt hatte. In den DIN-Stilen behaelt address auch hier seine normale
%%  Bedeutung als "Verlagsort" bei!
%%  In einigen entry-types werden zu Gunsten bibliographischer Vollstaendigkeit
%%  mehr optionale Felder verwendet als seinerzeit von Patashnik angegeben.
%%  Treten "Schoenheitsfehler" im fertig gesetzten output auf,
%%  lassen sich diese so gut wie immer durch eine veraenderte
%%  Erfassung im bib-inputfile beseitigen. Oren Patashnik empfiehlt, die
%%  Definition der Felder weit auszulegen. Last but not least koennen
%%  Sie im output-file < *.bbl > noch letzte Hand zur Korrektur ansetzen.
%%  Wegen der meist langen Internetadressen kann es zu "unschoenen" Luecken
%%  im Belegtext kommen. Dann muss mit \underfull hbox.... gekaempft werden.
%%
%%  Die Darstellung von Internetadressen wird durch das Zusatzpaket
%%  url.sty  ver 3.1, 15-Mar-2004 von Donald Arseneau erheblich verbessert und
%%  wird sehr empfohlen.
%%
%%  HYPERREF-Paket: wird dieses Paket zusaetzlich geladen, werden im output
%%  aktivierbare externe (URLs usw.) und interne (Dokumentbezogene) Links
%%  gesetzt. Sehr gute Zusammenarbeit mit PDFLaTex u.a.
%
%%  WARN- UND FEHLERMELDUNGEN
%%  Ursache von Warnmeldungen sind meistens ausgelassene Felder oder
%%  Erfassungs-"Fehler". Letztere haengen teilweise mit den gegenueber US-
%%  Gepflogenheiten andersartigen bibliographischen Regeln nach DIN 1505
%%  zusammen. Sie sind also in Wahrheit keine "Fehler" und duerfen fast immer
%%  ignoriert werden. Dennoch pruefen Sie diese Warnungen, um heraus zu finden,
%%  ob Publikationstyp (=entry-type) und "fields" eventuell unzulaessig
%%  kombiniert worden sind.
%%  Echte Fehler ("errors") duerften nur noch bei bibliographisch falscher
%%  Erfassung auftreten. Pruefen Sie die Syntax, den entry-type und die fields.
%%  Zu guter letzt: Qualitaetsmasstab ist einzig der DIN-konforme output!
%%
%%  DANKSAGUNG
%%  Hartmut Lueddecke, HAW Hamburg, hat viele Verbesserungsvorschlaege
%%  in die frueheren Versionen eingebracht. Ihm danke ich herzlich.
%%  Patrick W. Daly, dem Entwickler des Natbib-Stils, verdanke ich viele
%%  Anregungen und den steten Ansporn, die DIN-Stile zu verbessern.
%%  Helge Baumann hatte mit seiner Weiterentwicklung meines alten natdin.bst
%%  zu dinat.bst (Vers. 2001) die volle Zitierkapazitaet des natbib-Pakets
%%  eingefuehrt. Damit war ein deutlicher Zugewinn erreicht. Von ihm stammt
%%  der in der vorliegenden natdin.bst-Version 3.0x neu eingefuehrte Befehl
%%  \dinatlabel unter seinem von H. Baumann vergebenen Namen.
%%  Viele an dieser Stelle ungenannt bleibende Anwender haben mich in
%%  den vergangenen Jahren auf Fehler oder Verbesserungsmoeglichkeiten
%%  aufmerksam gemacht und so diesen Stil mitentwickelt. Ihnen gilt mein
%%  besonderer Dank. Ihr Feedback ist immer willkommen und eine Ermunterung.
%%
%%  Klaus F. Lorenzen
%%
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%  version 0.99c for BibTeX versions 0.99c or later, LaTeX2e version
%%  Copyright (C) 1985, all rights reserved.
%%  Copying of this file is authorized only if either
%%  (1) you make absolutely no changes to your copy, including name, or
%%  (2) if you do make changes, you name it something other than
%%  natdin.bst, natbib.sty
%%  This restriction helps ensure that all standard styles are identical.
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%
%%  NEUE FELDER
%%  Zur Erfassung von Internetquellen, E-mail u.a. gibt es folgende
%%  neue Felder: doi, lastchecked (nach Gray), url, urn
%%  Internetquellen (z.B. auch E-mail) werden vorzugsweise mit dem
%%  BOOKLET-Typ erfasst.
%%  Normen, Patente, Schutzrechte, Gesetzesstellen  sind mit dem MISC-Typ
%%  zu erfassen.
%%


ENTRY
  { address      %%  Verlagsort (immer!)
    author       %%  persoenlicher Urheber eines Werkes oder am Zustandekommen
                 %%  beteiligte Personen(=Mitarbeiter, Uebersetzer, Redakteur u.a.)
    booktitle    %%  a) Gesamttitel eines mehrbaendigen Werkes
%                %%  b) Titel des Sammelwerks, das einzelne selbstaendige
%                %%     Beitraege mit eigenem Titel enthaelt ->incollection
    chapter      %%  Kapitel in einem Buch (Monographie)
    doi          %%% Digital Object Identifier ->article
    edition      %%  a) Auflagevermerk
%                %%  b) bei selbst. elektron. Quellen == Version ->booklet
    editor       %%  Persoenl.Herausgeber oder Koerperschaftlicher Herausgeber
    howpublished %%  beliebiger Verlegervermerk: veroeffentlicht "von wem, wo"
    institution  %%  Institution, die e.verlagsfreie Veroeffentlichung betreibt
    isbn         %%  Standardnr fuer Buecher
    issn         %%  - " -    :      Zeitschriften u. Serien
    journal      %%  Titel einer Zeitschrift
    key          %%  Zusaetzlich vergebener Sortierschluessel, mitunter notwend.
    lastchecked  %%  neues Feld fuer das Datum des Online-Abrufs
%                %%  einer Internetquelle (n. GRAY )
    month        %%  naehere Bestimmung des Erscheinungsjahres -> macro 's
    note         %%  freies Eingabefeld fuer zusaetzliche Informationen z. Quelle
    number       %%  Versch. Bedeutungen in Abhaengigkeit vom Eingabetyp:
%                %%  a) Bandnummer einer gezaehlten Reihe (series)
%                %%  b) Heftnummer einer Zeitschrift ->article
%                %%  c) Nummer eines Forschungsberichts ->techreport
    organization %%  a) Name der Organisation/des Organisators e. Tagung,Konferenz
%                %%  b) Name einer Firma/Gesellschaft, die ein ->manual herausgab
    pages        %%  Umfangsangaben, meist Seitenzahlen
    publisher    %%  Verlag
    school       %%  Hochschule/Universitaet, die eine Dipl.-Arb./Dissertation veroeff.
    series       %%  Titel e.Reihe, in der ein best. Buchtitel erschienen ist
    title        %%  Titel einer (namentlich gekennzeichneten) Veroeffentlichung
    type         %%  Zusatzfeld z.Kennzeichnung e.besonderen Publikationstyps
    url          %%  neues Feld URL ( Uniform Resource Locator ):
%                %%  Serveradresse einer Internetquelle
    urn          %%  neues Feld URN ( Uniform Resource Name ):
%                %%  Persistent Identifier einer Internetquelle
    volume       %%  a) Zaehlung bei einem mehrbaendigen Werk ->book/->proceedings
%                %%  b) Jahrgang einer Zeitschrift ->article
    year         %%  Erscheinungsjahr
  }
  {}
  { label extra.label sort.label short.list dinat.label}

%%%----------------------------------------------------------------------------
%  Einige Standardvorgaben, die vom Benutzer veraendert werden koennen.
%%%----------------------------------------------------------------------------

%  Abkuerzung ("... und andere") bei Mehrverfasserquellen:

FUNCTION { ua.etal } { " et~al." }  %% evtl. auch in eckigen Klammern  " [u.\,a.]"

%%  oder lateinisch:  FUNCTION { ua.etal } { " et~al." }

FUNCTION { und } { " \& " }

%%  oder ausgeschrieben:  FUNCTION { und } { " und " }


% Einige elektronische Medien erhalten nach DIN 1505 eine "Ergaenzende Angabe"
% zusaetzlich zum materiellen Typ, z.B. CD ROM oder DVD u.a.:

FUNCTION { eress } { "Elektronische Ressource" }
%%%-----------------------------------------------------------------------------------

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

INTEGERS { after.firstblock }

INTEGERS { colon.after  period.dash }

INTEGERS { zahl  lang }

INTEGERS { len }

INTEGERS { longest.label.width last.extra.num number.label }

INTEGERS { nameptr namesleft numnames }

INTEGERS { ptr collation collrest }

STRINGS { longest.label last.label next.extra }

STRINGS { h s t u v w }

STRINGS { fkt }

%%---------------------------

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
  #4 'colon.after :=
  #5 'period.dash :=
  #6 'after.firstblock :=
}



FUNCTION {set.period.dash}    %% Wenn ein ". - " die Satzteile trennen soll.!
{ output.state before.all =
    'skip$
    { period.dash  'output.state := }
  if$
}


FUNCTION {set.period.dash.check}
{ empty$
    'skip$
    'set.period.dash
  if$
}

FUNCTION {set.colon.after}   %%$$$ Wenn ein ": " d. Satzteile trennen soll!
{ output.state before.all =
    'skip$
    { colon.after 'output.state  := }
  if$
}

%%           Wenn ein " " die Satzteile trennen soll.!
FUNCTION {new.sentence}
{ output.state before.all =
     'skip$
     { after.sentence 'output.state := }
  if$
}

%% neu 17/2/94                 Wenn ein ", " die Satzteile trennen soll.!
FUNCTION { part.of.sentence }
{ output.state before.all =
     'skip$
     { mid.sentence 'output.state := }
  if$
}

FUNCTION {new.sentence.checka}
{ empty$
    'skip$
    'new.sentence
  if$
}

FUNCTION {output.nonnull}
{ 's :=
  output.state after.block =
      { add.period$  write$
        newline$
        "\newblock " write$
      }
      { output.state before.all =
          { write$ }
          {  output.state colon.after =
               { ": " * write$
                 newline$
                 "\newblock " write$
               }
               { output.state period.dash =
                   { ". -- " *  write$
                     newline$
                     "\newblock " write$
                   }
                   { output.state mid.sentence =
                       { ", " * write$ }
                       { output.state after.sentence =
                           { " " * write$ }
                           { output.state after.firstblock =
                               { add.period$  write$
                                 newline$
                                 "\newblock " write$
                               }
                               { write$
                                 newline$
                                 "\newblock " write$
                               }
                             if$
                            }
                          if$
                       }
                     if$
                   }
                 if$
               }
             if$
           }
         if$
       after.block 'output.state :=
      }
    if$
    s
 }

FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}

FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}

FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}

FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}

FUNCTION {format.date}
{ year duplicate$ empty$
    { "empty year in " cite$ * warning$
       pop$ "" }
     'skip$
  if$
  month empty$
     'skip$
    { type$ "book" =
      type$ "inbook" =
       OR
         'skip$
         { month " " * swap$ * }
      if$
     }
   if$
%%  ohne Extrabuchstabe beim Erscheinungsjahr
}

FUNCTION {format.edition.or.date}
{ edition empty$ year empty$ and
    { "" }
    { edition empty$
        { type empty$ NOT
            { type #-1 #4 substring$ "mail" =
              type #1 #4 substring$ "Mail" =
              OR
                { " gesendet: " "-- " type * swap$ *
                  format.date *
                }
                { "\,Version:\,"
                  format.date *
                }
              if$
             }
             { "\,Version:\,"
               format.date *
             }
           if$
        }
        { year empty$
            { "\,Version:\," edition * }
            { "\,Version:\," edition * ", " *
              format.date *
            }
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.online.lastcheck}
{ lastchecked empty$
      { url empty$ doi empty$ urn empty$ and and
          { skip$ }
          { "" output }
        if$
      }
      { url empty$ doi empty$ urn empty$ and and
          { "there's a lastchecked date but no url, urn or doi in "
             cite$ * warning$
          }
          { part.of.sentence
            lastchecked "Abruf: " swap$ * output
          }
        if$
      }
    if$
}

FUNCTION {format.maillist.lastcheck}
   { type empty$ NOT
       { type #-1 #4 substring$ "mail" =
         type #1 #4 substring$ "Mail" =
         OR
           { format.online.lastcheck }
           'skip$
         if$
       }
       'skip$ 
     if$
   }

FUNCTION {format.doi}
{ doi empty$
    { "" }
    { new.block "\url{http://dx.doi.org/" doi * "}" *
     %%      { new.block "\url{http://dx.medra.org/" doi * "}" *
    }
  if$
}

FUNCTION {format.url}
{ urn missing$
     { doi missing$
          { url empty$
             { "" }
             { ""
             }
           if$
          }
          { "" }
        if$
      }
      { "" }
    if$
}

FUNCTION {format.maillist.url}
  { url empty$
       { "" }
       { type empty$ 
             { "" }
             { type #-1 #4 substring$ "mail" =
               type #1 #4 substring$ "Mail" =
               OR
                  { "\url{" url * "}" * }
                  { "" }
                if$
              }
           if$
        }
      if$
   }


FUNCTION {format.full.names}
{'s :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}" format.name$ 't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              t "others" =
                { ua.etal * }
                { und * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {author.editor.full}
{ author empty$
    { editor empty$
        { "" }
        { editor format.full.names }
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {author.full}
{ author empty$
    { "" }
    { author format.full.names }
  if$
}

FUNCTION {editor.full}
{ editor empty$
    { "" }
    { editor format.full.names }
  if$
}

FUNCTION {make.full.names}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.full
    { type$ "proceedings" =
        'editor.full
        'author.full
      if$
    }
  if$
}


FUNCTION {output.bibitem}
{ newline$
  "\bibitem[" write$
  label write$
  ")" make.full.names duplicate$ short.list =
     { pop$ }
     { * }
   if$
  "]{" * write$
  cite$ write$
  "}" write$
  newline$
  "\dinatlabel{" dinat.label * "} " *   %% Zeilenumbruch steht in NATBIB.CFG!
  write$
  ""
  before.all 'output.state :=
}


FUNCTION {fin.entry}
{ write$
  newline$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}

FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "\emph{" swap$ * "}" * }
  if$
}

FUNCTION { capitalize }
 { duplicate$ empty$
    { pop$ "" }
    { "\textsc{" swap$ * "}" * }
  if$
}

FUNCTION {article.in.journal}
{ duplicate$ empty$
    { pop$ "" }
    { author missing$ title missing$ and
            { emphasize }
            { emphasize "{}" swap$ * }
          if$
     }
  if$
}

FUNCTION {format.names}
{ 's :=
  "" 'u  :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    {
       s nameptr "{ll}" format.name$ 't :=
       t capitalize 't :=
       s nameptr "{ jj}" format.name$ 'w :=
       s nameptr "{, ff}{ vv}{ jj}" format.name$ 'u :=
       u  text.length$  'lang :=
       #1 'zahl :=
       "" 'v :=
         {  zahl  lang  <  }
           {  u  zahl  #1  substring$  "~"  =
               {  v  ""  =
                     {  u  #1  zahl  #1  -  substring$  'v :=  }
                     'skip$
                  if$
                  v  u  zahl  #2  substring$ * "." *  w * 'v :=
                }
                'skip$
              if$
            zahl  #1  +  'zahl :=  }
      while$
      v  ""  =
         {  u  'v :=  }
         'skip$
      if$
      t  v  *  fkt  *  't :=
      nameptr #1 >
         {
          nameptr #3
          #1 + =
          numnames #4
          > and
            { "et~al." 't :=
              #1 'namesleft := }
            'skip$
          if$
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              numnames #2 >
                  { "" * }
                  'skip$
               if$
               t "\textsc{others}" = t "\textsc{others} (Hrsg.)" = or
                  { ua.etal * }
                  { ", " * t * }
               if$
               }
            if$  %% Ende der namesleft-Pruefung
          }
            't
           if$  %%  Ende der nameptr-Pruefung

      nameptr #1 + 'nameptr :=
      namesleft #1 -  'namesleft :=
    }
  while$  %%  Ende von { namesleft #0 > } ganz oben
  "" 'fkt :=  %% fkt wird zurueckgesetzt
}

FUNCTION {format.authors}
{ author empty$
    { "" }
    { author format.names }
  if$
}

FUNCTION {format.editors}
{ editor empty$
   { author empty$
       { "empty author and editor in " cite$ * warning$ "" }
       'skip$
     if$
   }
   { author empty$
        { " (Hrsg.)" 'fkt :=
          editor format.names
        }
        { " (Hrsg.)" 'fkt :=
          " ; " * editor format.names *
        }
      if$
   }
 if$
 }

%%  2005-11-11
FUNCTION { format.authors.organization }
{ type$ "misc" =
        { organization empty$
            { author empty$
               { "" }
               { author format.names " (Erfinder)" * }
             if$
            }
            { author empty$
               { organization  }
               { author format.names " (Erfinder); " *
                 organization * " (Anmelder)" *
               }
             if$
            }
          if$
        }
        { type$ "manual" =
           { organization empty$
               { format.authors }
               { author empty$
                   { organization capitalize " (Hrsg.)" * }
                   { author format.names }
                 if$
               }
             if$
           }
           'skip$
         if$
        }
      if$     
}

FUNCTION { format.editors.organization }
{ organization empty$
    'skip$
    { type$ "misc" =
        { organization }
        { * " ; " * organization " (Veranst.)" *}
      if$
    }
  if$
}

FUNCTION { format.tr.institution }
{ institution empty$
    'skip$
   { institution capitalize }
 if$
}

FUNCTION {format.ed.incoll}
{ editor empty$
     { "" }
     { " (Hrsg.)" 'fkt :=
       editor format.names
       format.editors.organization
     }
  if$
}


FUNCTION {format.title}
{ title empty$
    { "" }
    { title }  %% Text so wie er dasteht im Feld title
  if$
}

FUNCTION {format.number}
{ number empty$
    { "" }
    { number " " * }  %% Text so wie er im Feld number steht plus " "
  if$
}

FUNCTION {format.digital.type}
{ type empty$
    { "" }
    { type #-1 #4 substring$ "mail" =
      type #1 #4 substring$ "Mail" =
      OR
        { "" }
        { type }  %% Typ einer digitalen Ressource in Form einer
              %% "Ergaenzenden Angabe", so wie er dasteht;
              %% Alternativ kann dieser Text auch in NOTE erfasst werden.
      if$
    }
 if$
}

FUNCTION {n.dashify}
{ 't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

%%  Auflagenvermerke gibt man komplett, einschliesslich Abkuerzungen in
%%  das Feld edition ein: ---> EDITION= { 3., erw. und verb. Aufl. }
%%  oder fremdsprachlich:      EDITION= { 2nd edition }

FUNCTION {format.edition}
{ edition empty$
    { "" }
    { edition }
  if$
}

FUNCTION {format.version.url}
{ url empty$ doi empty$ urn empty$ and and
   { type$ "techreport" =
       { format.edition }
       { "" }
     if$
   }
   { format.edition.or.date output format.url }
 if$
}

FUNCTION {format.edition.or.version}
{ url empty$ doi empty$ urn empty$ and and
   { format.edition }
   { format.edition.or.date }
 if$
}

FUNCTION {format.address.publisher.year}
{  publisher empty$
      { address empty$
          { year empty$
              { "" }
              { year }
            if$
          }
          { "there's an address but no publisher in " cite$ * warning$
              address ", " * format.date *
          }
        if$
      }
      { address empty$
          { year empty$
              { "neither address nor publication date in " cite$ * warning$
                 publisher
              }
              { publisher ", " * format.date * }
            if$
          }
          { year empty$
              { address " : " * publisher * }
              { address " : " * publisher * ", " * format.date * }
            if$
          }
        if$
       }
     if$
}

FUNCTION {format.howpublished}
{ url missing$ urn missing$ doi missing$ AND AND
    { howpublished empty$
        { address empty$
            { type empty$
              { "" }
              { type #-1 #4 substring$ "mail" =
                  { "(gesendet: " new.sentence
                    format.date * ")" *
                  }
                  { "" }
                if$
               }
             if$
             format.date *
            }
            { address ", " * format.date * }
          if$
        }
        { address empty$
            { howpublished ", " * format.date * }
            { address " : " * howpublished * ", " * format.date * }
          if$
        }
      if$
    }
    { howpublished empty$
        { "" }
        { howpublished }
      if$
    }
  if$
}

FUNCTION {format.btitle}
{ title emphasize
}

FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$ * *
}

FUNCTION {format.btitle.vol}
{ number empty$
   { series empty$
     { volume empty$
        { title emphasize }
        { title emphasize ". Bd." * volume tie.or.space.connect }
       if$
     }
     { volume empty$
        { title emphasize }%% ein Buch, das zusaetzl. SERIES=Reihentitel besitzt
    %% jetzt kommt d. Fall des mehrbaendigen Werkes mit Gesamttitel=SERIES
    %% Zaehlung=VOLUME und Bandtitel=TITLE;
        { series emphasize ". Bd." * volume tie.or.space.connect
                                 ": " * "{\emph{" * title * "}}" * }
       if$
     }
     if$%% series-test
   }
   { title emphasize }%% wenn number ex., dann immer title-Feld
  if$%% Ende number-test
}

FUNCTION {format.series.number.din}
{ volume empty$
    { number empty$
          { series empty$
               { "" }
               { "(" series * ")" * } %% d. Seriennr koennte auch gleich hier
                                      %% im SERIES-Feld miterfasst werden
            if$
          }
          { series empty$
               { "(" number tie.or.space.connect ")" *
                 "there's a number but no series in " cite$ * warning$
               }
               { "(" series * number tie.or.space.connect ")" * }
            if$
          }
       if$
     }
     { series empty$
          { "" }
          { type$ "proceedings" =  %% Sonderfall, es darf VOLUME und NUMBER ex. !
            type$ "inproceedings" = OR
                { number empty$
                    { "(" series * ")" * }
                    { "(" series * number tie.or.space.connect ")" * }
                  if$
                }
                { "" }%%   Ausstieg mit Nullstring, s. Kommentar
            if$
          }%% bei gezaehlten Reihen MUSS die Reihennr. im Feld NUMBER stehen!
       if$ %% wenn also d. Feld VOLUME nicht leer ist, dann liegt ausser bei
           %% Typ PROCEEDINGS/INPROCEEDINGS falsche
      }     %% Erfassung vor und es erfolgt d. Ausstieg mit d. Nullstring!
  if$
}

FUNCTION {format.tr.series.or.number}
{    number empty$
       { series empty$
           { "" }
           { "(" series * ")" * }
         if$
       }
       { series empty$
         { "(" number * ")" * }
         { "(" series * number tie.or.space.connect ")" * }
       if$
       }
     if$
 }

FUNCTION {format.misc.series}
{ series empty$
    { "" }
    { "(" series * ")" * }
  if$
}

FUNCTION { format.doi.urn }
{ urn empty$
     { doi empty$
          { "" }
          { "" }
       if$
     }
     { "" }
  if$
}

FUNCTION { format.isbn.issn }
{ isbn empty$
     { issn empty$
          { "" }
          { "" }
       if$
     }
     { "" }
  if$
}

FUNCTION {format.pages}
{ pages empty$
    { "" }
    { url empty$
        { "S." pages n.dashify  tie.or.space.connect }
        { pages }
      if$
    }
  if$
}

FUNCTION {format.pages.book}
{ pages empty$
    { "" }
    { note empty$ isbn empty$ AND
         { "" pages n.dashify tie.or.space.connect " S" *
           add.period$
         }
         { "" pages n.dashify tie.or.space.connect " S" *
         }
       if$
     }
  if$
}

FUNCTION {format.pages.bkcollation}
{ pages empty$
    { "" }
    { "" pages n.dashify tie.or.space.connect }
  if$
}

FUNCTION {format.bkpages.collat.check}
{ 's :=
  #1 'ptr :=
  s text.length$ 'collation :=
   collation #1 =
    { format.pages.book }
    { 
      collation 'collrest :=
       { collrest #0 > }
       { s ptr #2 substring$ 't :=
         t "S." =
           { format.pages.bkcollation
             #0 'collrest := }
           { ptr #1 + 'ptr :=
             collrest #1 - 'collrest :=
             #1 collrest =
               { format.pages.book }
               { skip$ }
             if$
           }
         if$
       }
       while$
    }
  if$
}

FUNCTION {format.vol.year.num.pages}
{ volume field.or.null
    year empty$
      { "there's no year in " cite$ * warning$ }
      { " (" year * ")" * * }
    if$
    month empty$
      'skip$
      { ", " month * * }
    if$
    number empty$
      'skip$
      { ", Nr. " number * * }
    if$
    pages empty$
      'skip$
      { duplicate$ empty$
        { pop$ "" }
        { title missing$
            { ", " pages format.bkpages.collat.check * *}
            { ", " format.pages * *}
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.chapter.inbook}
{ duplicate$  empty$
    { pop$ "empty chapter in " cite$ * warning$ }
    { type empty$
         { "\emph{Kapitel\/} " swap$ tie.or.space.connect }
         { type " " * swap$ * }%%  wenn keine bes. Abschnittsform gen. werden soll,
                 %%  koennte e. kl. Zwischenraum gewaehlt werden, z.B. " \, "
       if$
     }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
        { "Kapitel " }
        { url empty$
           { type }
           { "Kapitel " }
         if$
        }
      if$
      chapter tie.or.space.connect
      pages empty$
         'skip$
        { ", " * format.pages * }
      if$
     }
  if$
}

FUNCTION {format.in.ed.booktitle.din}
{ booktitle empty$
    { "" }
    { editor empty$
        { volume empty$
            { "{In: }" booktitle emphasize * }%% n. Belieben fettes In:
            { "{In: }" booktitle emphasize *  %%      - " -
              " Bd." volume tie.or.space.connect *
            }
          if$
        }
        { volume empty$
            { "{In: }" format.ed.incoll * ": " * booktitle emphasize * }
            { "{In: }" format.ed.incoll * ": " * booktitle emphasize *
              " Bd." volume tie.or.space.connect *
            }
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.thesis.tr.type}
{ type empty$
    'skip$
   { pop$
     type
   }
 if$
}

FUNCTION {format.article.crossref}
{ key empty$
    { journal empty$
        { "need key or journal for " cite$ * " to crossref " * crossref *
          warning$
          ""
        }
        { "{In: }{\emph " journal * "}" * }%% n. Belieben fettes In:
      if$
    }
    { "{In: }" key * }%%    s.o. fettes In:
  if$
  " {\textbf{\citep{" * crossref * "}" * "}" * "}" * ", " * format.pages *
}

FUNCTION {format.crossref.editor}
%vorher,Lue  { editor #1 "{vv~}{ll}" format.name$ " (Hrsg.)" *
 { editor #1 "{ll}" format.name$ " (Hrsg.)" *
   editor num.names$ duplicate$
   #2 >
    { pop$ ua.etal * }
    { #2 <
        'skip$
        { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            { ua.etal * }
            { " ; " * editor #2 "{vv~}{ll}" format.name$ * " (Hrsg.)" * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.inbk.vol.title}
{ volume empty$
     { " In: " }
     { title empty$
        { " In: Bd." volume tie.or.space.connect
                " von " *
        }
        { "In: Bd." volume tie.or.space.connect ": " * title emphasize *
                     " (" * year * ") in " *
        }
      if$
     }
   if$
 }

FUNCTION {format.book.crossref}
{ type$ "inbook" =
   { format.inbk.vol.title }
   { volume empty$
       { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
         " "
       }
       { ". -- Bd." volume tie.or.space.connect
          " von " *
       }
     if$
    }
  if$
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
        { series empty$
            { "need editor, key, or series for " cite$ * " to crossref " *
              crossref * warning$
              "" *
            }
            { "" * }%% dadurch kommt nach der Band Nr. gleich das label 2/6/99
%%              { "{\emph{" * series * "}} {\textbf{siehe}} " * }
          if$
        }
        { key * }
      if$
    }
    { "" * }
  if$
  "{\textbf{\citep{" * crossref * "}" * "}" * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
    editor field.or.null author field.or.null =
    or
     { key empty$
        { booktitle empty$
            { "need editor, key, or booktitle for " cite$ * " to crossref " *
              crossref * warning$
              ""
            }
            { "{In: }{\emph " booktitle * "}" * }%%
          if$
        }
        { "{In: }" }
      if$
     }
    { "{In: }" }
  if$
  "{\textbf{\citep{" * crossref * "}" * "}" * "}" * %% ", " * format.pages *
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.title "title" output.check
  crossref missing$
    { journal article.in.journal output.nonnull
      new.sentence
      format.vol.year.num.pages output
      format.url output
    }
    { format.article.crossref output.nonnull }
  if$
  format.online.lastcheck
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  issn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors format.editors output.nonnull }
  if$
  set.colon.after
  crossref missing$
    { format.btitle.vol "title" output.check }
    { format.btitle "title" output.check }
  if$
  format.edition output
  format.address.publisher.year "publisher" output.check
  new.sentence
  crossref missing$
    { format.series.number.din output }
    { format.book.crossref output.nonnull }
  if$
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  format.doi output
  format.url output
  new.block
  isbn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {booklet}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors format.editors output.nonnull }
  if$
  set.colon.after
  format.btitle "title" output.check
  format.edition.or.version output
  format.url output
  format.online.lastcheck
  format.howpublished output
  series new.sentence.checka
  format.series.number.din output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  type set.period.dash.check
  format.digital.type output
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  note set.period.dash.check
  note output
  format.isbn.issn output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
    chapter format.chapter.inbook output.nonnull
      crossref missing$
      { author empty$
          { format.editors "\,{In:\,}" swap$ * "author and editor" output.check }
          { format.authors "\,{In:\,}" swap$ * output.nonnull }
        if$
        author empty$ editor empty$ AND
           { before.all 'output.state := }
           { set.colon.after }
         if$
      format.btitle.vol "title" output.check
      format.edition output
      format.address.publisher.year "publisher" output.check
      new.sentence
      format.series.number.din output
      isbn set.period.dash.check
      format.isbn.issn output
    }
    { format.book.crossref output.nonnull
    }
  if$
    part.of.sentence
    format.pages output
    note set.period.dash.check
    note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.title "title" output.check
  format.version.url output
  type empty$ NOT
      { type #-1 #4 substring$ "mail" =
        type #1 #4 substring$ "Mail" =
        OR
           'skip$
           { format.online.lastcheck }
        if$
      }
      { format.online.lastcheck }    
   if$
  crossref missing$
    { format.in.ed.booktitle.din "booktitle" output.check
      format.edition output 
      format.address.publisher.year "publisher" output.check
      format.maillist.url output
      format.maillist.lastcheck
      new.sentence
      format.series.number.din output
      doi set.period.dash.check
      urn set.period.dash.check
      format.doi.urn output
      isbn set.period.dash.check
      issn set.period.dash.check
      format.isbn.issn output
    }
    { format.incoll.inproc.crossref output.nonnull }
  if$
  part.of.sentence
  format.chapter.pages "pages" output.check
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.title "title" output.check
  crossref missing$
    { format.in.ed.booktitle.din "booktitle" output.check
      address empty$
        { organization new.sentence.checka
          organization output
          part.of.sentence
          format.address.publisher.year output
        }
        { format.address.publisher.year "publisher" output.check }
      if$
      new.sentence
      format.series.number.din output
      isbn set.period.dash.check
      issn set.period.dash.check
      format.isbn.issn output
      format.url output  %TB210717: added url for proc
    }
    { format.incoll.inproc.crossref output.nonnull }
  if$
      part.of.sentence
      format.pages output
      note set.period.dash.check
      note output
      fin.entry
}

FUNCTION {conference} { inproceedings }%% nach Patashnik, wg US-Kompatibilitaet

FUNCTION {manual}
{ output.bibitem
  author empty$
    { organization empty$
        { title empty$
            'skip$
            {format.btitle "title" output.check }
          if$
        }
        'skip$
      if$
    }
    'skip$
  if$
  format.authors.organization output.nonnull
  set.colon.after
  format.btitle "title" output.check
  format.edition "edition" output.check
  author empty$ organization empty$ AND
    {   address "address" output.check
        part.of.sentence
    }
    { organization empty$
        { address "address" output.check
          part.of.sentence
        }
        { address ": " * organization * output
          part.of.sentence
        }
      if$
    }
  if$
  format.date output
  number empty$
    'skip$
   { "(" number * ") " * output }
  if$
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  format.doi output
  format.url output
  format.online.lastcheck
  note set.period.dash.check
  note output
  fin.entry
}

%%  Standard ist "Diplomarbeit", anderes mit TYPE="anderer Typ" erfassen!
%%  z.B. TYPE={Hausarbeit}, TYPE={Diss.}, TYPE={Habil.}, TYPE={Magisterarb.}
FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.btitle "title" output.check
  address output
  part.of.sentence
  school "school" output.check
  part.of.sentence
  "Diplomarbeit" format.thesis.tr.type output.nonnull
  part.of.sentence
  format.date "year" output.check
  format.url output
  format.online.lastcheck
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {phdthesis} %%  {mastersthesis}% ist identisch bis auf Standardwert, s.o.
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.btitle "title" output.check
  address output
  part.of.sentence
  school "school" output.check
  part.of.sentence
  "Diss." format.thesis.tr.type output.nonnull % koennte auch `Dissertation' sein
  part.of.sentence
  format.date "year" output.check
  format.url output
  format.online.lastcheck
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  note set.period.dash.check
  note output
  fin.entry
}


%% Normen, Vornormen, Schutzrechte (Patente) werden hiermit erfasst;
%% E-mail, (auch Internetressourcen moeglich; besser --> booklet-Fkt!)
%% das type-Feld uebernimmt eine wichtige Steuerfunktion:
FUNCTION {misc}
{ output.bibitem
   type missing$ not
       { type duplicate$ #1 #4 substring$ "Norm" =
           type #1 #4 substring$ "Vorn" = OR
           { " " *
             format.number * output
             new.sentence
             format.date output
             title empty$
               { skip$ }
               { add.period$ new.sentence }
             if$
             format.btitle "title" output.check
             note set.period.dash.check
             note output
           }
           { duplicate$ #1 #6 substring$ "Schutz" =
                { " " * format.number * output
                  new.sentence
                  "(" * format.date ")" * output
                  add.period$ new.sentence
                  format.authors.organization add.period$ output
                  note output
                }
            %%  wenn irgendein anderer Typ eingetragen ist
                { pop$ pop$ ""
                  title empty$
                     { note empty$
                         { url empty$
                             { "there's no relevant field in " cite$ warning$
                                pop$ ""
                             }
                             { format.url output }%%%
                           if$
                         }
                         { note " " * output.nonnull }
                       if$
                     }
                     { author empty$
                          { editor empty$
                               { organization empty$
                                   { skip$ }
                                   { format.editors.organization output.nonnull
                                     set.colon.after
                                   }
                                 if$
                               }
                               { format.editors format.editors.organization
                                 output.nonnull set.colon.after
                               }
                             if$
                          }
                          { format.authors format.editors output.nonnull
                            set.colon.after
                          }
                        if$
                 format.btitle output.nonnull
                 url empty$
                   { format.edition output
                     format.howpublished output}
                   { format.howpublished output
                     format.edition.or.version output
                     format.url output
                   }
                 if$
                 format.online.lastcheck
                 new.sentence
                 format.misc.series output
                 note set.period.dash.check
                 note output
                }
              if$
            }
         if$
          }
        if$
       }
       %% wenn es keinen type gibt
       { title empty$
             { note empty$
                 { url empty$
                     { "there's no relevant field in " cite$ warning$
                       pop$ ""
                     }
                     { format.url output }%%%  das waere e. reine URL
                   if$
                 }
                 { note " " * output.nonnull
                 }
               if$
             }
             { author empty$
                   { editor empty$
                        { organization empty$
                             'skip$
                             { format.editors.organization output.nonnull
                               set.colon.after
                             }
                           if$
                        }
                        { format.editors format.editors.organization
                          output.nonnull set.colon.after
                        }
                      if$
                   }
                   { format.authors format.editors output.nonnull
                     set.colon.after
                   }
                 if$
              format.btitle output.nonnull
              url empty$
                { format.edition output
                  format.howpublished output}
                { format.howpublished output
                  format.url output
                  format.edition.or.date output
                  format.online.lastcheck
                }
              if$
              new.sentence
              format.misc.series output
              note set.period.dash.check
              note output
          }
        if$
      }
    if$
 fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
    editor empty$
      { organization empty$
           { "empty organization and editor in " cite$ * warning$ }
           { organization " (Veranst.)" * output }
        if$
      }
      { format.editors format.editors.organization output.nonnull }
    if$
  set.colon.after
  format.btitle "title" output.check
  volume empty$
    'skip$
    { "{\textnormal{Bd.}}" volume tie.or.space.connect emphasize "volume" output.check }
  if$
  format.address.publisher.year "publisher" output.check
  new.sentence
  format.series.number.din output.nonnull
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  isbn set.period.dash.check
  issn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      format.tr.institution output.nonnull }
    { format.authors  format.editors output.nonnull }
  if$
  set.colon.after
  format.title "title" output.check
  institution empty$
     'skip$
    { author empty$ editor empty$ AND
          'skip$
        { institution new.sentence.checka
          "/ " institution *  output.nonnull
        }
      if$
    }
  if$
  format.version.url output
  format.online.lastcheck
  format.address.publisher.year output
  number new.sentence.checka
  format.tr.series.or.number "number" output.check
  "Forschungsbericht" format.thesis.tr.type set.period.dash.check
  "Forschungsbericht" format.thesis.tr.type output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  isbn set.period.dash.check
  issn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note "note" output.check
  fin.entry
}


FUNCTION {unpublished} {misc}%% author, title, note muessen sein! howpublished
%%                           %% entfaellt natuerlich

FUNCTION {default.type} { misc }

MACRO {jan} {"Januar"}

MACRO {feb} {"Februar"}

MACRO {mar} {"M{\^^b a}rz"}

MACRO {apr} {"April"}

MACRO {mai} {"Mai"}

MACRO {may} {"Mai"}

MACRO {jun} {"Juni"}

MACRO {jul} {"Juli"}

MACRO {aug} {"August"}

MACRO {sep} {"September"}

MACRO {okt} {"Oktober"}

MACRO {oct} {"Oktober"}

MACRO {nov} {"November"}

MACRO {dez} {"Dezember"}

MACRO {dec} {"Dezember"}

%%$$$  stillgelegte Beispiele fuer den Gebrauch von Kuerzeln (hier Zs-Titel).

%%MACRO {acmcs} {"ACM Computing Surveys"}

%%MACRO {acta} {"Acta Informatica"}

READ

FUNCTION {sortify}
{ purify$
  "l" change.case$
}

FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}

FUNCTION {format.lab.names}
{ 's :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$ ua.etal * }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            { ua.etal * }
            { und * s #2 "{vv~}{ll}" format.name$ * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { year empty$
           'key
           { editor format.lab.names }
         if$
        }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.key.organization.label}
{ author empty$
    { key empty$
        { organization empty$
            { cite$ #1 #3 substring$ }
            { "The " #4 organization chop.word #3 text.prefix$ }
          if$
        }
        { key }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.organization.label}
{ editor empty$
    { key empty$
        { organization empty$
            { cite$ #1 #3 substring$ }
            { "The " #4 organization chop.word #4 text.prefix$ }
          if$
        }
        { key }
      if$
    }
    { key empty$%%  das key-feld soll zwangsweise das label machen!
        { editor format.lab.names }
        { key }%%das ganze label
      if$
    }
  if$
}
FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "booklet" =
  type$ "inbook" =
  or or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.organization.label
        { type$ "manual" =
            'author.key.organization.label
            'author.key.label
          if$
        }
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  "("
  *
%%  year duplicate$ empty$
%%  short.list key field.or.null = or
%%      { pop$ "" }
%%      'skip$
%%   if$
  year field.or.null purify$ #1 #4 substring$
  *
  'label :=
  short.list " " *
  year field.or.null purify$ #1 #4 substring$ * 'dinat.label :=
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { nameptr #1 >
        { "   " * }
        'skip$
      if$
      s nameptr "{ll{ }}{  ff{ }}{ vv{ }}{  jj{ }}" format.name$ 't :=
      nameptr numnames = t "others" = and
        { ua.etal * }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "Der " #4
        "Die " #4
          "Das " #4
            "Ein " #4
              "Eine " #5
                  "The " #4 t chop.word
               chop.word
             chop.word
           chop.word
         chop.word
       chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.organization.sort}
{ author empty$
    { organization empty$
        { key empty$
            { "to sort, need author, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {editor.organization.sort.PWD}%% so war es in plainnat
{ editor empty$
    { organization empty$
        { key empty$
            { "to sort, need editor, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { editor sort.format.names }
  if$
}

FUNCTION {editor.organization.sort}%%das key-Feld soll z. Sortieren ben. werden
{ key empty$
    { editor empty$
       { organization empty$
            { "to sort, need editor, organization, or key in " cite$ * warning$
             ""
            }
            { "The " #4 organization chop.word sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { key sortify }
  if$
}

FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "booklet" =
  type$ "inbook" =
  or or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.organization.sort
        { type$ "manual" =
            'author.organization.sort
            'author.sort
          if$
        }
      if$
    }
  if$
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.label :=
  sort.label *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}

SORT

FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'longest.label.width :=
  #0 'last.extra.num :=
  #0 'number.label :=
}

FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}

FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
  label extra.label * 'label :=
  dinat.label extra.label * 'dinat.label :=
}

EXECUTE {initialize.longest.label}

ITERATE {forward.pass}

REVERSE {reverse.pass}

FUNCTION {bib.sort.order}
{ sort.label  'sort.key$ :=
}

ITERATE {bib.sort.order}

SORT

FUNCTION {begin.bib}
{   preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" *
  write$ newline$ newline$
  "% this bibliography is generated by nd24.bst [3.0c2] from 2005-12-21"
  write$ newline$ newline$
  "\providecommand{\natexlab}[1]{#1}"
  write$ newline$
  "\providecommand{\url}[1]{\texttt{#1}}"
  write$ newline$
  "\makeatletter"
  write$ newline$
  "\newcommand{\dinatlabel}[1]%"
  write$ newline$
  "{\ifNAT@numbers\else\NAT@biblabelnum{#1}\fi}"
  write$ newline$
  "\makeatother"
  write$ newline$
  "\expandafter\ifx\csname urlstyle\endcsname\relax"
  write$ newline$
  "  \providecommand{\doi}[1]{doi: #1}\else"
  write$ newline$
  "  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi"
  write$ newline$
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}

==> natdin_et_al.tex <==
%%  natdin.bst   Vers. [3.1]  2006-01-02   mit PWD cite-multimode
%%
%%  Aenderungen seit Vers. [3.0bx]:
%%  a) Funktions-Zusaetze bei Autoren sind nun moeglich
%%  b) Internetquellen ohne Zusatz "Online--Ressource" !
%%  c) verbesserte INPROCEEDINGS, PROCEEDINGS-Funktionen
%%  d) neue TECHREPORT und MANUAL-Funktionen
%%  e) neue format.pages.book-Funktion
%%  f) neue format.online.lastchecked-Funktion
%%  
%%
%%   K.F.Lorenzen  (Copyright 1994-2006)  email:  lorenzen.marxen@t-online.de
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%  Mit diesem BibTex-style werden Literaturverzeichnisse nach dem deutschen
%%  Standard DIN 1505, Teil 2 und 3 formatiert. Die label im Quellen-/
%%  Literaturverzeichnis sind vom Typ 'Verfasser - Jahr' und
%%  entsprechen den Zitatformen im Text. Es koennen alle von
%%  Patrick W. Daly im natbib-Paket implementierten Zitierbefehle
%%  genutzt werden. Eine Kurzbeschreibung liegt als Datei natnotes.pdf zusammen
%%  mit der im Aufbau befindlichen Beschreibung des natdin-Stils
%%  unter der URL  http://www.haw-hamburg.de/pers/Lorenzen/bibtex.
%%  Eine Anleitung zur Anwendung der Norm DIN 1505 findet sich unter der
%%  URL http://www.bui.haw-hamburg.de/pers/klaus.lorenzen/ASP/litverz.pdf
%%
%%  Es werden nun auch Elektronische Online / Offline Ressourcen wie
%%  Internetquellen, CD-ROM usw. verarbeitet. Dazu kommen spezielle
%%  Publikationsformen wie Patente, Normen, Karten, Fernsehaufzeichnungen,
%%  Gesetzesstellen, Spiele u.a.
%
%%  NATDIN.BST muss zusammen mit NATBIB.STY von Patrick W. Daly und der in
%%  dieser Verteilung modifizierten Konfiguration NATBIB.CFG aufgerufen
%%  werden. NATDIN.BST ist vorzugsweise in den ...\bibtex\bst - Pfad zu
%%  stellen. Die jeweils individuelle Konfiguration NATBIB.CFG wird am
%%  besten in das Verzeichnis der LaTex-Quelle selbst gelegt.
%%
%%  Eine Muster-Konfiguration wird auf Vorschlag von Helge Baumann eingefuegt:
%   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%   NATBIB.CFG        in Verbindung mit natbib.sty     Lorenzen, 2005-05-31
%		      diese Konfigurationsdatei wird zuletzt eingelesen und
%		      enthaelt die lokal gewuenschten Einstellungen fuer den
%		      Bibliographie-- und Zitierstil
%
%   \newcommand{\bibstyle@natdin}%
%       {\bibpunct{(}{)}{;}{a}{}{,~}
%       \gdef\NAT@biblabelnum##1{\textbf{##1}\\}} %% \\ bewirkt Zeilenumbruch
%                                                 %% nach label-Ausgabe
%
%   \bibstyle@natdin
%
%   % Einzug der Belege nach der Einordnungsmarke
%   \setlength{\bibhang}{7mm}
%
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%
%%  Zur Gewaehrleistung der Allgemeingueltigkeit von bib-files gelten
%%  in den DIN-styles mit einer einzigen Ausnahme die in der Tex-Literatur
%%  veroeffentlichten originalen Definitionen und Regeln fuer die
%%  Publikationstypen (entry-types) und die bibliographischen Felder (fields).
%%  Die Ausnahme bezieht sich auf den entry-type PROCEEDINGS und das Feld
%%  address, fuer das Oren Patashnik dort die Sonderbedeutung "Konferenzort"
%%  gewaehlt hatte. In den DIN-Stilen behaelt address auch hier seine normale
%%  Bedeutung als "Verlagsort" bei!
%%  In einigen entry-types werden zu Gunsten bibliographischer Vollstaendigkeit
%%  mehr optionale Felder verwendet als seinerzeit von Patashnik angegeben.
%%  Treten "Schoenheitsfehler" im fertig gesetzten output auf,
%%  lassen sich diese so gut wie immer durch eine veraenderte
%%  Erfassung im bib-inputfile beseitigen. Oren Patashnik empfiehlt, die
%%  Definition der Felder weit auszulegen. Last but not least koennen
%%  Sie im output-file < *.bbl > noch letzte Hand zur Korrektur ansetzen.
%%  Wegen der meist langen Internetadressen kann es zu "unschoenen" Luecken
%%  im Belegtext kommen. Dann muss mit \underfull hbox.... gekaempft werden.
%%
%%  Die Darstellung von Internetadressen wird durch das Zusatzpaket
%%  url.sty  ver 3.1, 15-Mar-2004 von Donald Arseneau erheblich verbessert und
%%  wird sehr empfohlen.
%%
%%  HYPERREF-Paket: wird dieses Paket zusaetzlich geladen, werden im output
%%  aktivierbare externe (URLs usw.) und interne (Dokumentbezogene) Links
%%  gesetzt. Sehr gute Zusammenarbeit mit PDFLaTex u.a.
%
%%  WARN- UND FEHLERMELDUNGEN
%%  Ursache von Warnmeldungen sind meistens ausgelassene Felder oder
%%  Erfassungs-"Fehler". Letztere haengen teilweise mit den gegenueber US-
%%  Gepflogenheiten andersartigen bibliographischen Regeln nach DIN 1505
%%  zusammen. Sie sind also in Wahrheit keine "Fehler" und duerfen fast immer
%%  ignoriert werden. Dennoch pruefen Sie diese Warnungen, um heraus zu finden,
%%  ob Publikationstyp (=entry-type) und "fields" eventuell unzulaessig
%%  kombiniert worden sind.
%%  Echte Fehler ("errors") duerften nur noch bei bibliographisch falscher
%%  Erfassung auftreten. Pruefen Sie die Syntax, den entry-type und die fields.
%%  Zu guter letzt: Qualitaetsmasstab ist einzig der DIN-konforme output!
%%
%%  DANKSAGUNG
%%  Hartmut Lueddecke, HAW Hamburg, hat viele Verbesserungsvorschlaege
%%  in die frueheren Versionen eingebracht. Ihm danke ich herzlich.
%%  Patrick W. Daly, dem Entwickler des Natbib-Stils, verdanke ich viele
%%  Anregungen und den steten Ansporn, die DIN-Stile zu verbessern.
%%  Helge Baumann hatte mit seiner Weiterentwicklung meines alten natdin.bst
%%  zu dinat.bst (Vers. 2001) die volle Zitierkapazitaet des natbib-Pakets
%%  eingefuehrt. Damit war ein deutlicher Zugewinn erreicht. Von ihm stammt
%%  der in der vorliegenden natdin.bst-Version 3.0x neu eingefuehrte Befehl
%%  \dinatlabel unter seinem von H. Baumann vergebenen Namen.
%%  Viele an dieser Stelle ungenannt bleibende Anwender haben mich in
%%  den vergangenen Jahren auf Fehler oder Verbesserungsmoeglichkeiten
%%  aufmerksam gemacht und so diesen Stil mitentwickelt. Ihnen gilt mein
%%  besonderer Dank. Ihr Feedback ist immer willkommen und eine Ermunterung.
%%
%%  Klaus F. Lorenzen
%%
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%  version 0.99c for BibTeX versions 0.99c or later, LaTeX2e version
%%  Copyright (C) 1985, all rights reserved.
%%  Copying of this file is authorized only if either
%%  (1) you make absolutely no changes to your copy, including name, or
%%  (2) if you do make changes, you name it something other than
%%  natdin.bst, natbib.sty
%%  This restriction helps ensure that all standard styles are identical.
%%  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%
%%  NEUE FELDER
%%  Zur Erfassung von Internetquellen, E-mail u.a. gibt es folgende
%%  neue Felder: doi, lastchecked (nach Gray), url, urn
%%  Internetquellen (z.B. auch E-mail) werden vorzugsweise mit dem
%%  BOOKLET-Typ erfasst.
%%  Normen, Patente, Schutzrechte, Gesetzesstellen  sind mit dem MISC-Typ
%%  zu erfassen.
%%


ENTRY
  { address      %%  Verlagsort (immer!)
    author       %%  persoenlicher Urheber eines Werkes oder am Zustandekommen
                 %%  beteiligte Personen(=Mitarbeiter, Uebersetzer, Redakteur u.a.)
    booktitle    %%  a) Gesamttitel eines mehrbaendigen Werkes
%                %%  b) Titel des Sammelwerks, das einzelne selbstaendige
%                %%     Beitraege mit eigenem Titel enthaelt ->incollection
    chapter      %%  Kapitel in einem Buch (Monographie)
    doi          %%% Digital Object Identifier ->article
    edition      %%  a) Auflagevermerk
%                %%  b) bei selbst. elektron. Quellen == Version ->booklet
    editor       %%  Persoenl.Herausgeber oder Koerperschaftlicher Herausgeber
    howpublished %%  beliebiger Verlegervermerk: veroeffentlicht "von wem, wo"
    institution  %%  Institution, die e.verlagsfreie Veroeffentlichung betreibt
    isbn         %%  Standardnr fuer Buecher
    issn         %%  - " -    :      Zeitschriften u. Serien
    journal      %%  Titel einer Zeitschrift
    key          %%  Zusaetzlich vergebener Sortierschluessel, mitunter notwend.
    lastchecked  %%  neues Feld fuer das Datum des Online-Abrufs
%                %%  einer Internetquelle (n. GRAY )
    month        %%  naehere Bestimmung des Erscheinungsjahres -> macro 's
    note         %%  freies Eingabefeld fuer zusaetzliche Informationen z. Quelle
    number       %%  Versch. Bedeutungen in Abhaengigkeit vom Eingabetyp:
%                %%  a) Bandnummer einer gezaehlten Reihe (series)
%                %%  b) Heftnummer einer Zeitschrift ->article
%                %%  c) Nummer eines Forschungsberichts ->techreport
    organization %%  a) Name der Organisation/des Organisators e. Tagung,Konferenz
%                %%  b) Name einer Firma/Gesellschaft, die ein ->manual herausgab
    pages        %%  Umfangsangaben, meist Seitenzahlen
    publisher    %%  Verlag
    school       %%  Hochschule/Universitaet, die eine Dipl.-Arb./Dissertation veroeff.
    series       %%  Titel e.Reihe, in der ein best. Buchtitel erschienen ist
    title        %%  Titel einer (namentlich gekennzeichneten) Veroeffentlichung
    type         %%  Zusatzfeld z.Kennzeichnung e.besonderen Publikationstyps
    url          %%  neues Feld URL ( Uniform Resource Locator ):
%                %%  Serveradresse einer Internetquelle
    urn          %%  neues Feld URN ( Uniform Resource Name ):
%                %%  Persistent Identifier einer Internetquelle
    volume       %%  a) Zaehlung bei einem mehrbaendigen Werk ->book/->proceedings
%                %%  b) Jahrgang einer Zeitschrift ->article
    year         %%  Erscheinungsjahr
  }
  {}
  { label extra.label sort.label short.list dinat.label}

%%%----------------------------------------------------------------------------
%  Einige Standardvorgaben, die vom Benutzer veraendert werden koennen.
%%%----------------------------------------------------------------------------

%  Abkuerzung ("... und andere") bei Mehrverfasserquellen:

FUNCTION { ua.etal } { " et~al." }  %% evtl. auch in eckigen Klammern  " [u.\,a.]"

%%  oder lateinisch:  FUNCTION { ua.etal } { " et~al." }

FUNCTION { und } { " \& " }

%%  oder ausgeschrieben:  FUNCTION { und } { " und " }


% Einige elektronische Medien erhalten nach DIN 1505 eine "Ergaenzende Angabe"
% zusaetzlich zum materiellen Typ, z.B. CD ROM oder DVD u.a.:

FUNCTION { eress } { "Elektronische Ressource" }
%%%-----------------------------------------------------------------------------------

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

INTEGERS { after.firstblock }

INTEGERS { colon.after  period.dash }

INTEGERS { zahl  lang }

INTEGERS { len }

INTEGERS { longest.label.width last.extra.num number.label }

INTEGERS { nameptr namesleft numnames }

INTEGERS { ptr collation collrest }

STRINGS { longest.label last.label next.extra }

STRINGS { h s t u v w }

STRINGS { fkt }

%%---------------------------

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
  #4 'colon.after :=
  #5 'period.dash :=
  #6 'after.firstblock :=
}



FUNCTION {set.period.dash}    %% Wenn ein ". - " die Satzteile trennen soll.!
{ output.state before.all =
    'skip$
    { period.dash  'output.state := }
  if$
}


FUNCTION {set.period.dash.check}
{ empty$
    'skip$
    'set.period.dash
  if$
}

FUNCTION {set.colon.after}   %%$$$ Wenn ein ": " d. Satzteile trennen soll!
{ output.state before.all =
    'skip$
    { colon.after 'output.state  := }
  if$
}

%%           Wenn ein " " die Satzteile trennen soll.!
FUNCTION {new.sentence}
{ output.state before.all =
     'skip$
     { after.sentence 'output.state := }
  if$
}

%% neu 17/2/94                 Wenn ein ", " die Satzteile trennen soll.!
FUNCTION { part.of.sentence }
{ output.state before.all =
     'skip$
     { mid.sentence 'output.state := }
  if$
}

FUNCTION {new.sentence.checka}
{ empty$
    'skip$
    'new.sentence
  if$
}

FUNCTION {output.nonnull}
{ 's :=
  output.state after.block =
      { add.period$  write$
        newline$
        "\newblock " write$
      }
      { output.state before.all =
          { write$ }
          {  output.state colon.after =
               { ": " * write$
                 newline$
                 "\newblock " write$
               }
               { output.state period.dash =
                   { ". -- " *  write$
                     newline$
                     "\newblock " write$
                   }
                   { output.state mid.sentence =
                       { ", " * write$ }
                       { output.state after.sentence =
                           { " " * write$ }
                           { output.state after.firstblock =
                               { add.period$  write$
                                 newline$
                                 "\newblock " write$
                               }
                               { write$
                                 newline$
                                 "\newblock " write$
                               }
                             if$
                            }
                          if$
                       }
                     if$
                   }
                 if$
               }
             if$
           }
         if$
       after.block 'output.state :=
      }
    if$
    s
 }

FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}

FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}

FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}

FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}

FUNCTION {format.date}
{ year duplicate$ empty$
    { "empty year in " cite$ * warning$
       pop$ "" }
     'skip$
  if$
  month empty$
     'skip$
    { type$ "book" =
      type$ "inbook" =
       OR
         'skip$
         { month " " * swap$ * }
      if$
     }
   if$
%%  ohne Extrabuchstabe beim Erscheinungsjahr
}

FUNCTION {format.edition.or.date}
{ edition empty$ year empty$ and
    { "" }
    { edition empty$
        { type empty$ NOT
            { type #-1 #4 substring$ "mail" =
              type #1 #4 substring$ "Mail" =
              OR
                { " gesendet: " "-- " type * swap$ *
                  format.date *
                }
                { "\,Version:\,"
                  format.date *
                }
              if$
             }
             { "\,Version:\,"
               format.date *
             }
           if$
        }
        { year empty$
            { "\,Version:\," edition * }
            { "\,Version:\," edition * ", " *
              format.date *
            }
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.online.lastcheck}
{ lastchecked empty$
      { url empty$ doi empty$ urn empty$ and and
          { skip$ }
          { "" output }
        if$
      }
      { url empty$ doi empty$ urn empty$ and and
          { "there's a lastchecked date but no url, urn or doi in "
             cite$ * warning$
          }
          { part.of.sentence
            lastchecked "Abruf: " swap$ * output
          }
        if$
      }
    if$
}

FUNCTION {format.maillist.lastcheck}
   { type empty$ NOT
       { type #-1 #4 substring$ "mail" =
         type #1 #4 substring$ "Mail" =
         OR
           { format.online.lastcheck }
           'skip$
         if$
       }
       'skip$ 
     if$
   }

FUNCTION {format.doi}
{ doi empty$
    { "" }
    { new.block "\url{http://dx.doi.org/" doi * "}" *
     %%      { new.block "\url{http://dx.medra.org/" doi * "}" *
    }
  if$
}

FUNCTION {format.url}
{ urn missing$
     { doi missing$
          { url empty$
             { "" }
             { ""
             }
           if$
          }
          { "" }
        if$
      }
      { "" }
    if$
}

FUNCTION {format.maillist.url}
  { url empty$
       { "" }
       { type empty$ 
             { "" }
             { type #-1 #4 substring$ "mail" =
               type #1 #4 substring$ "Mail" =
               OR
                  { "\url{" url * "}" * }
                  { "" }
                if$
              }
           if$
        }
      if$
   }


FUNCTION {format.full.names}
{'s :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}" format.name$ 't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              t "others" =
                { ua.etal * }
                { und * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {author.editor.full}
{ author empty$
    { editor empty$
        { "" }
        { editor format.full.names }
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {author.full}
{ author empty$
    { "" }
    { author format.full.names }
  if$
}

FUNCTION {editor.full}
{ editor empty$
    { "" }
    { editor format.full.names }
  if$
}

FUNCTION {make.full.names}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.full
    { type$ "proceedings" =
        'editor.full
        'author.full
      if$
    }
  if$
}


FUNCTION {output.bibitem}
{ newline$
  "\bibitem[" write$
  label write$
  ")" make.full.names duplicate$ short.list =
     { pop$ }
     { * }
   if$
  "]{" * write$
  cite$ write$
  "}" write$
  newline$
  "\dinatlabel{" dinat.label * "} " *   %% Zeilenumbruch steht in NATBIB.CFG!
  write$
  ""
  before.all 'output.state :=
}


FUNCTION {fin.entry}
{ write$
  newline$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}

FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "\emph{" swap$ * "}" * }
  if$
}

FUNCTION { capitalize }
 { duplicate$ empty$
    { pop$ "" }
    { "\textsc{" swap$ * "}" * }
  if$
}

FUNCTION {article.in.journal}
{ duplicate$ empty$
    { pop$ "" }
    { author missing$ title missing$ and
            { emphasize }
            { emphasize "{}" swap$ * }
          if$
     }
  if$
}

FUNCTION {format.names}
{ 's :=
  "" 'u  :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    {
       s nameptr "{ll}" format.name$ 't :=
       t capitalize 't :=
       s nameptr "{ jj}" format.name$ 'w :=
       s nameptr "{, ff}{ vv}{ jj}" format.name$ 'u :=
       u  text.length$  'lang :=
       #1 'zahl :=
       "" 'v :=
         {  zahl  lang  <  }
           {  u  zahl  #1  substring$  "~"  =
               {  v  ""  =
                     {  u  #1  zahl  #1  -  substring$  'v :=  }
                     'skip$
                  if$
                  v  u  zahl  #2  substring$ * "." *  w * 'v :=
                }
                'skip$
              if$
            zahl  #1  +  'zahl :=  }
      while$
      v  ""  =
         {  u  'v :=  }
         'skip$
      if$
      t  v  *  fkt  *  't :=
      nameptr #1 >
         {
          nameptr #3
          #1 + =
          numnames #4
          > and
            { "et~al." 't :=
              #1 'namesleft := }
            'skip$
          if$
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              numnames #2 >
                  { "" * }
                  'skip$
               if$
               t "\textsc{others}" = t "\textsc{others} (Hrsg.)" = or
                  { ua.etal * }
                  { ", " * t * }
               if$
               }
            if$  %% Ende der namesleft-Pruefung
          }
            't
           if$  %%  Ende der nameptr-Pruefung

      nameptr #1 + 'nameptr :=
      namesleft #1 -  'namesleft :=
    }
  while$  %%  Ende von { namesleft #0 > } ganz oben
  "" 'fkt :=  %% fkt wird zurueckgesetzt
}

FUNCTION {format.authors}
{ author empty$
    { "" }
    { author format.names }
  if$
}

FUNCTION {format.editors}
{ editor empty$
   { author empty$
       { "empty author and editor in " cite$ * warning$ "" }
       'skip$
     if$
   }
   { author empty$
        { " (Hrsg.)" 'fkt :=
          editor format.names
        }
        { " (Hrsg.)" 'fkt :=
          " ; " * editor format.names *
        }
      if$
   }
 if$
 }

%%  2005-11-11
FUNCTION { format.authors.organization }
{ type$ "misc" =
        { organization empty$
            { author empty$
               { "" }
               { author format.names " (Erfinder)" * }
             if$
            }
            { author empty$
               { organization  }
               { author format.names " (Erfinder); " *
                 organization * " (Anmelder)" *
               }
             if$
            }
          if$
        }
        { type$ "manual" =
           { organization empty$
               { format.authors }
               { author empty$
                   { organization capitalize " (Hrsg.)" * }
                   { author format.names }
                 if$
               }
             if$
           }
           'skip$
         if$
        }
      if$     
}

FUNCTION { format.editors.organization }
{ organization empty$
    'skip$
    { type$ "misc" =
        { organization }
        { * " ; " * organization " (Veranst.)" *}
      if$
    }
  if$
}

FUNCTION { format.tr.institution }
{ institution empty$
    'skip$
   { institution capitalize }
 if$
}

FUNCTION {format.ed.incoll}
{ editor empty$
     { "" }
     { " (Hrsg.)" 'fkt :=
       editor format.names
       format.editors.organization
     }
  if$
}


FUNCTION {format.title}
{ title empty$
    { "" }
    { title }  %% Text so wie er dasteht im Feld title
  if$
}

FUNCTION {format.number}
{ number empty$
    { "" }
    { number " " * }  %% Text so wie er im Feld number steht plus " "
  if$
}

FUNCTION {format.digital.type}
{ type empty$
    { "" }
    { type #-1 #4 substring$ "mail" =
      type #1 #4 substring$ "Mail" =
      OR
        { "" }
        { type }  %% Typ einer digitalen Ressource in Form einer
              %% "Ergaenzenden Angabe", so wie er dasteht;
              %% Alternativ kann dieser Text auch in NOTE erfasst werden.
      if$
    }
 if$
}

FUNCTION {n.dashify}
{ 't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

%%  Auflagenvermerke gibt man komplett, einschliesslich Abkuerzungen in
%%  das Feld edition ein: ---> EDITION= { 3., erw. und verb. Aufl. }
%%  oder fremdsprachlich:      EDITION= { 2nd edition }

FUNCTION {format.edition}
{ edition empty$
    { "" }
    { edition }
  if$
}

FUNCTION {format.version.url}
{ url empty$ doi empty$ urn empty$ and and
   { type$ "techreport" =
       { format.edition }
       { "" }
     if$
   }
   { format.edition.or.date output format.url }
 if$
}

FUNCTION {format.edition.or.version}
{ url empty$ doi empty$ urn empty$ and and
   { format.edition }
   { format.edition.or.date }
 if$
}

FUNCTION {format.address.publisher.year}
{  publisher empty$
      { address empty$
          { year empty$
              { "" }
              { year }
            if$
          }
          { "there's an address but no publisher in " cite$ * warning$
              address ", " * format.date *
          }
        if$
      }
      { address empty$
          { year empty$
              { "neither address nor publication date in " cite$ * warning$
                 publisher
              }
              { publisher ", " * format.date * }
            if$
          }
          { year empty$
              { address " : " * publisher * }
              { address " : " * publisher * ", " * format.date * }
            if$
          }
        if$
       }
     if$
}

FUNCTION {format.howpublished}
{ url missing$ urn missing$ doi missing$ AND AND
    { howpublished empty$
        { address empty$
            { type empty$
              { "" }
              { type #-1 #4 substring$ "mail" =
                  { "(gesendet: " new.sentence
                    format.date * ")" *
                  }
                  { "" }
                if$
               }
             if$
             format.date *
            }
            { address ", " * format.date * }
          if$
        }
        { address empty$
            { howpublished ", " * format.date * }
            { address " : " * howpublished * ", " * format.date * }
          if$
        }
      if$
    }
    { howpublished empty$
        { "" }
        { howpublished }
      if$
    }
  if$
}

FUNCTION {format.btitle}
{ title emphasize
}

FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$ * *
}

FUNCTION {format.btitle.vol}
{ number empty$
   { series empty$
     { volume empty$
        { title emphasize }
        { title emphasize ". Bd." * volume tie.or.space.connect }
       if$
     }
     { volume empty$
        { title emphasize }%% ein Buch, das zusaetzl. SERIES=Reihentitel besitzt
    %% jetzt kommt d. Fall des mehrbaendigen Werkes mit Gesamttitel=SERIES
    %% Zaehlung=VOLUME und Bandtitel=TITLE;
        { series emphasize ". Bd." * volume tie.or.space.connect
                                 ": " * "{\emph{" * title * "}}" * }
       if$
     }
     if$%% series-test
   }
   { title emphasize }%% wenn number ex., dann immer title-Feld
  if$%% Ende number-test
}

FUNCTION {format.series.number.din}
{ volume empty$
    { number empty$
          { series empty$
               { "" }
               { "(" series * ")" * } %% d. Seriennr koennte auch gleich hier
                                      %% im SERIES-Feld miterfasst werden
            if$
          }
          { series empty$
               { "(" number tie.or.space.connect ")" *
                 "there's a number but no series in " cite$ * warning$
               }
               { "(" series * number tie.or.space.connect ")" * }
            if$
          }
       if$
     }
     { series empty$
          { "" }
          { type$ "proceedings" =  %% Sonderfall, es darf VOLUME und NUMBER ex. !
            type$ "inproceedings" = OR
                { number empty$
                    { "(" series * ")" * }
                    { "(" series * number tie.or.space.connect ")" * }
                  if$
                }
                { "" }%%   Ausstieg mit Nullstring, s. Kommentar
            if$
          }%% bei gezaehlten Reihen MUSS die Reihennr. im Feld NUMBER stehen!
       if$ %% wenn also d. Feld VOLUME nicht leer ist, dann liegt ausser bei
           %% Typ PROCEEDINGS/INPROCEEDINGS falsche
      }     %% Erfassung vor und es erfolgt d. Ausstieg mit d. Nullstring!
  if$
}

FUNCTION {format.tr.series.or.number}
{    number empty$
       { series empty$
           { "" }
           { "(" series * ")" * }
         if$
       }
       { series empty$
         { "(" number * ")" * }
         { "(" series * number tie.or.space.connect ")" * }
       if$
       }
     if$
 }

FUNCTION {format.misc.series}
{ series empty$
    { "" }
    { "(" series * ")" * }
  if$
}

FUNCTION { format.doi.urn }
{ urn empty$
     { doi empty$
          { "" }
          { "" }
       if$
     }
     { "" }
  if$
}

FUNCTION { format.isbn.issn }
{ isbn empty$
     { issn empty$
          { "" }
          { "" }
       if$
     }
     { "" }
  if$
}

FUNCTION {format.pages}
{ pages empty$
    { "" }
    { url empty$
        { "S." pages n.dashify  tie.or.space.connect }
        { pages }
      if$
    }
  if$
}

FUNCTION {format.pages.book}
{ pages empty$
    { "" }
    { note empty$ isbn empty$ AND
         { "" pages n.dashify tie.or.space.connect " S" *
           add.period$
         }
         { "" pages n.dashify tie.or.space.connect " S" *
         }
       if$
     }
  if$
}

FUNCTION {format.pages.bkcollation}
{ pages empty$
    { "" }
    { "" pages n.dashify tie.or.space.connect }
  if$
}

FUNCTION {format.bkpages.collat.check}
{ 's :=
  #1 'ptr :=
  s text.length$ 'collation :=
   collation #1 =
    { format.pages.book }
    { 
      collation 'collrest :=
       { collrest #0 > }
       { s ptr #2 substring$ 't :=
         t "S." =
           { format.pages.bkcollation
             #0 'collrest := }
           { ptr #1 + 'ptr :=
             collrest #1 - 'collrest :=
             #1 collrest =
               { format.pages.book }
               { skip$ }
             if$
           }
         if$
       }
       while$
    }
  if$
}

FUNCTION {format.vol.year.num.pages}
{ volume field.or.null
    year empty$
      { "there's no year in " cite$ * warning$ }
      { " (" year * ")" * * }
    if$
    month empty$
      'skip$
      { ", " month * * }
    if$
    number empty$
      'skip$
      { ", Nr. " number * * }
    if$
    pages empty$
      'skip$
      { duplicate$ empty$
        { pop$ "" }
        { title missing$
            { ", " pages format.bkpages.collat.check * *}
            { ", " format.pages * *}
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.chapter.inbook}
{ duplicate$  empty$
    { pop$ "empty chapter in " cite$ * warning$ }
    { type empty$
         { "\emph{Kapitel\/} " swap$ tie.or.space.connect }
         { type " " * swap$ * }%%  wenn keine bes. Abschnittsform gen. werden soll,
                 %%  koennte e. kl. Zwischenraum gewaehlt werden, z.B. " \, "
       if$
     }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
        { "Kapitel " }
        { url empty$
           { type }
           { "Kapitel " }
         if$
        }
      if$
      chapter tie.or.space.connect
      pages empty$
         'skip$
        { ", " * format.pages * }
      if$
     }
  if$
}

FUNCTION {format.in.ed.booktitle.din}
{ booktitle empty$
    { "" }
    { editor empty$
        { volume empty$
            { "{In: }" booktitle emphasize * }%% n. Belieben fettes In:
            { "{In: }" booktitle emphasize *  %%      - " -
              " Bd." volume tie.or.space.connect *
            }
          if$
        }
        { volume empty$
            { "{In: }" format.ed.incoll * ": " * booktitle emphasize * }
            { "{In: }" format.ed.incoll * ": " * booktitle emphasize *
              " Bd." volume tie.or.space.connect *
            }
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.thesis.tr.type}
{ type empty$
    'skip$
   { pop$
     type
   }
 if$
}

FUNCTION {format.article.crossref}
{ key empty$
    { journal empty$
        { "need key or journal for " cite$ * " to crossref " * crossref *
          warning$
          ""
        }
        { "{In: }{\emph " journal * "}" * }%% n. Belieben fettes In:
      if$
    }
    { "{In: }" key * }%%    s.o. fettes In:
  if$
  " {\textbf{\citep{" * crossref * "}" * "}" * "}" * ", " * format.pages *
}

FUNCTION {format.crossref.editor}
%vorher,Lue  { editor #1 "{vv~}{ll}" format.name$ " (Hrsg.)" *
 { editor #1 "{ll}" format.name$ " (Hrsg.)" *
   editor num.names$ duplicate$
   #2 >
    { pop$ ua.etal * }
    { #2 <
        'skip$
        { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            { ua.etal * }
            { " ; " * editor #2 "{vv~}{ll}" format.name$ * " (Hrsg.)" * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {format.inbk.vol.title}
{ volume empty$
     { " In: " }
     { title empty$
        { " In: Bd." volume tie.or.space.connect
                " von " *
        }
        { "In: Bd." volume tie.or.space.connect ": " * title emphasize *
                     " (" * year * ") in " *
        }
      if$
     }
   if$
 }

FUNCTION {format.book.crossref}
{ type$ "inbook" =
   { format.inbk.vol.title }
   { volume empty$
       { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
         " "
       }
       { ". -- Bd." volume tie.or.space.connect
          " von " *
       }
     if$
    }
  if$
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
        { series empty$
            { "need editor, key, or series for " cite$ * " to crossref " *
              crossref * warning$
              "" *
            }
            { "" * }%% dadurch kommt nach der Band Nr. gleich das label 2/6/99
%%              { "{\emph{" * series * "}} {\textbf{siehe}} " * }
          if$
        }
        { key * }
      if$
    }
    { "" * }
  if$
  "{\textbf{\citep{" * crossref * "}" * "}" * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
    editor field.or.null author field.or.null =
    or
     { key empty$
        { booktitle empty$
            { "need editor, key, or booktitle for " cite$ * " to crossref " *
              crossref * warning$
              ""
            }
            { "{In: }{\emph " booktitle * "}" * }%%
          if$
        }
        { "{In: }" }
      if$
     }
    { "{In: }" }
  if$
  "{\textbf{\citep{" * crossref * "}" * "}" * "}" * %% ", " * format.pages *
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.title "title" output.check
  crossref missing$
    { journal article.in.journal output.nonnull
      new.sentence
      format.vol.year.num.pages output
      format.url output
    }
    { format.article.crossref output.nonnull }
  if$
  format.online.lastcheck
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  issn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors format.editors output.nonnull }
  if$
  set.colon.after
  crossref missing$
    { format.btitle.vol "title" output.check }
    { format.btitle "title" output.check }
  if$
  format.edition output
  format.address.publisher.year "publisher" output.check
  new.sentence
  crossref missing$
    { format.series.number.din output }
    { format.book.crossref output.nonnull }
  if$
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  format.doi output
  format.url output
  new.block
  isbn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {booklet}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors format.editors output.nonnull }
  if$
  set.colon.after
  format.btitle "title" output.check
  format.edition.or.version output
  format.url output
  format.online.lastcheck
  format.howpublished output
  series new.sentence.checka
  format.series.number.din output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  type set.period.dash.check
  format.digital.type output
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  note set.period.dash.check
  note output
  format.isbn.issn output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
    chapter format.chapter.inbook output.nonnull
      crossref missing$
      { author empty$
          { format.editors "\,{In:\,}" swap$ * "author and editor" output.check }
          { format.authors "\,{In:\,}" swap$ * output.nonnull }
        if$
        author empty$ editor empty$ AND
           { before.all 'output.state := }
           { set.colon.after }
         if$
      format.btitle.vol "title" output.check
      format.edition output
      format.address.publisher.year "publisher" output.check
      new.sentence
      format.series.number.din output
      isbn set.period.dash.check
      format.isbn.issn output
    }
    { format.book.crossref output.nonnull
    }
  if$
    part.of.sentence
    format.pages output
    note set.period.dash.check
    note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.title "title" output.check
  format.version.url output
  type empty$ NOT
      { type #-1 #4 substring$ "mail" =
        type #1 #4 substring$ "Mail" =
        OR
           'skip$
           { format.online.lastcheck }
        if$
      }
      { format.online.lastcheck }    
   if$
  crossref missing$
    { format.in.ed.booktitle.din "booktitle" output.check
      format.edition output 
      format.address.publisher.year "publisher" output.check
      format.maillist.url output
      format.maillist.lastcheck
      new.sentence
      format.series.number.din output
      doi set.period.dash.check
      urn set.period.dash.check
      format.doi.urn output
      isbn set.period.dash.check
      issn set.period.dash.check
      format.isbn.issn output
    }
    { format.incoll.inproc.crossref output.nonnull }
  if$
  part.of.sentence
  format.chapter.pages "pages" output.check
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.title "title" output.check
  crossref missing$
    { format.in.ed.booktitle.din "booktitle" output.check
      address empty$
        { organization new.sentence.checka
          organization output
          part.of.sentence
          format.address.publisher.year output
        }
        { format.address.publisher.year "publisher" output.check }
      if$
      new.sentence
      format.series.number.din output
      isbn set.period.dash.check
      issn set.period.dash.check
      format.isbn.issn output
      format.url output  %TB210717: added url for proc
    }
    { format.incoll.inproc.crossref output.nonnull }
  if$
      part.of.sentence
      format.pages output
      note set.period.dash.check
      note output
      fin.entry
}

FUNCTION {conference} { inproceedings }%% nach Patashnik, wg US-Kompatibilitaet

FUNCTION {manual}
{ output.bibitem
  author empty$
    { organization empty$
        { title empty$
            'skip$
            {format.btitle "title" output.check }
          if$
        }
        'skip$
      if$
    }
    'skip$
  if$
  format.authors.organization output.nonnull
  set.colon.after
  format.btitle "title" output.check
  format.edition "edition" output.check
  author empty$ organization empty$ AND
    {   address "address" output.check
        part.of.sentence
    }
    { organization empty$
        { address "address" output.check
          part.of.sentence
        }
        { address ": " * organization * output
          part.of.sentence
        }
      if$
    }
  if$
  format.date output
  number empty$
    'skip$
   { "(" number * ") " * output }
  if$
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  format.doi output
  format.url output
  format.online.lastcheck
  note set.period.dash.check
  note output
  fin.entry
}

%%  Standard ist "Diplomarbeit", anderes mit TYPE="anderer Typ" erfassen!
%%  z.B. TYPE={Hausarbeit}, TYPE={Diss.}, TYPE={Habil.}, TYPE={Magisterarb.}
FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.btitle "title" output.check
  address output
  part.of.sentence
  school "school" output.check
  part.of.sentence
  "Diplomarbeit" format.thesis.tr.type output.nonnull
  part.of.sentence
  format.date "year" output.check
  format.url output
  format.online.lastcheck
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {phdthesis} %%  {mastersthesis}% ist identisch bis auf Standardwert, s.o.
{ output.bibitem
  format.authors "author" output.check
  set.colon.after
  format.btitle "title" output.check
  address output
  part.of.sentence
  school "school" output.check
  part.of.sentence
  "Diss." format.thesis.tr.type output.nonnull % koennte auch `Dissertation' sein
  part.of.sentence
  format.date "year" output.check
  format.url output
  format.online.lastcheck
  doi set.period.dash.check
  urn set.period.dash.check
  format.doi.urn output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  note set.period.dash.check
  note output
  fin.entry
}


%% Normen, Vornormen, Schutzrechte (Patente) werden hiermit erfasst;
%% E-mail, (auch Internetressourcen moeglich; besser --> booklet-Fkt!)
%% das type-Feld uebernimmt eine wichtige Steuerfunktion:
FUNCTION {misc}
{ output.bibitem
   type missing$ not
       { type duplicate$ #1 #4 substring$ "Norm" =
           type #1 #4 substring$ "Vorn" = OR
           { " " *
             format.number * output
             new.sentence
             format.date output
             title empty$
               { skip$ }
               { add.period$ new.sentence }
             if$
             format.btitle "title" output.check
             note set.period.dash.check
             note output
           }
           { duplicate$ #1 #6 substring$ "Schutz" =
                { " " * format.number * output
                  new.sentence
                  "(" * format.date ")" * output
                  add.period$ new.sentence
                  format.authors.organization add.period$ output
                  note output
                }
            %%  wenn irgendein anderer Typ eingetragen ist
                { pop$ pop$ ""
                  title empty$
                     { note empty$
                         { url empty$
                             { "there's no relevant field in " cite$ warning$
                                pop$ ""
                             }
                             { format.url output }%%%
                           if$
                         }
                         { note " " * output.nonnull }
                       if$
                     }
                     { author empty$
                          { editor empty$
                               { organization empty$
                                   { skip$ }
                                   { format.editors.organization output.nonnull
                                     set.colon.after
                                   }
                                 if$
                               }
                               { format.editors format.editors.organization
                                 output.nonnull set.colon.after
                               }
                             if$
                          }
                          { format.authors format.editors output.nonnull
                            set.colon.after
                          }
                        if$
                 format.btitle output.nonnull
                 url empty$
                   { format.edition output
                     format.howpublished output}
                   { format.howpublished output
                     format.edition.or.version output
                     format.url output
                   }
                 if$
                 format.online.lastcheck
                 new.sentence
                 format.misc.series output
                 note set.period.dash.check
                 note output
                }
              if$
            }
         if$
          }
        if$
       }
       %% wenn es keinen type gibt
       { title empty$
             { note empty$
                 { url empty$
                     { "there's no relevant field in " cite$ warning$
                       pop$ ""
                     }
                     { format.url output }%%%  das waere e. reine URL
                   if$
                 }
                 { note " " * output.nonnull
                 }
               if$
             }
             { author empty$
                   { editor empty$
                        { organization empty$
                             'skip$
                             { format.editors.organization output.nonnull
                               set.colon.after
                             }
                           if$
                        }
                        { format.editors format.editors.organization
                          output.nonnull set.colon.after
                        }
                      if$
                   }
                   { format.authors format.editors output.nonnull
                     set.colon.after
                   }
                 if$
              format.btitle output.nonnull
              url empty$
                { format.edition output
                  format.howpublished output}
                { format.howpublished output
                  format.url output
                  format.edition.or.date output
                  format.online.lastcheck
                }
              if$
              new.sentence
              format.misc.series output
              note set.period.dash.check
              note output
          }
        if$
      }
    if$
 fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
    editor empty$
      { organization empty$
           { "empty organization and editor in " cite$ * warning$ }
           { organization " (Veranst.)" * output }
        if$
      }
      { format.editors format.editors.organization output.nonnull }
    if$
  set.colon.after
  format.btitle "title" output.check
  volume empty$
    'skip$
    { "{\textnormal{Bd.}}" volume tie.or.space.connect emphasize "volume" output.check }
  if$
  format.address.publisher.year "publisher" output.check
  new.sentence
  format.series.number.din output.nonnull
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  isbn set.period.dash.check
  issn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      format.tr.institution output.nonnull }
    { format.authors  format.editors output.nonnull }
  if$
  set.colon.after
  format.title "title" output.check
  institution empty$
     'skip$
    { author empty$ editor empty$ AND
          'skip$
        { institution new.sentence.checka
          "/ " institution *  output.nonnull
        }
      if$
    }
  if$
  format.version.url output
  format.online.lastcheck
  format.address.publisher.year output
  number new.sentence.checka
  format.tr.series.or.number "number" output.check
  "Forschungsbericht" format.thesis.tr.type set.period.dash.check
  "Forschungsbericht" format.thesis.tr.type output
  pages empty$
    { skip$ }
    { pages set.period.dash.check
      pages format.bkpages.collat.check output
    }
  if$
  isbn set.period.dash.check
  issn set.period.dash.check
  format.isbn.issn output
  note set.period.dash.check
  note "note" output.check
  fin.entry
}


FUNCTION {unpublished} {misc}%% author, title, note muessen sein! howpublished
%%                           %% entfaellt natuerlich

FUNCTION {default.type} { misc }

MACRO {jan} {"Januar"}

MACRO {feb} {"Februar"}

MACRO {mar} {"M{\^^b a}rz"}

MACRO {apr} {"April"}

MACRO {mai} {"Mai"}

MACRO {may} {"Mai"}

MACRO {jun} {"Juni"}

MACRO {jul} {"Juli"}

MACRO {aug} {"August"}

MACRO {sep} {"September"}

MACRO {okt} {"Oktober"}

MACRO {oct} {"Oktober"}

MACRO {nov} {"November"}

MACRO {dez} {"Dezember"}

MACRO {dec} {"Dezember"}

%%$$$  stillgelegte Beispiele fuer den Gebrauch von Kuerzeln (hier Zs-Titel).

%%MACRO {acmcs} {"ACM Computing Surveys"}

%%MACRO {acta} {"Acta Informatica"}

READ

FUNCTION {sortify}
{ purify$
  "l" change.case$
}

FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}

FUNCTION {format.lab.names}
{ 's :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$ ua.etal * }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            { ua.etal * }
            { und * s #2 "{vv~}{ll}" format.name$ * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { year empty$
           'key
           { editor format.lab.names }
         if$
        }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.key.organization.label}
{ author empty$
    { key empty$
        { organization empty$
            { cite$ #1 #3 substring$ }
            { "The " #4 organization chop.word #3 text.prefix$ }
          if$
        }
        { key }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.organization.label}
{ editor empty$
    { key empty$
        { organization empty$
            { cite$ #1 #3 substring$ }
            { "The " #4 organization chop.word #4 text.prefix$ }
          if$
        }
        { key }
      if$
    }
    { key empty$%%  das key-feld soll zwangsweise das label machen!
        { editor format.lab.names }
        { key }%%das ganze label
      if$
    }
  if$
}
FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "booklet" =
  type$ "inbook" =
  or or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.organization.label
        { type$ "manual" =
            'author.key.organization.label
            'author.key.label
          if$
        }
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  "("
  *
%%  year duplicate$ empty$
%%  short.list key field.or.null = or
%%      { pop$ "" }
%%      'skip$
%%   if$
  year field.or.null purify$ #1 #4 substring$
  *
  'label :=
  short.list " " *
  year field.or.null purify$ #1 #4 substring$ * 'dinat.label :=
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { nameptr #1 >
        { "   " * }
        'skip$
      if$
      s nameptr "{ll{ }}{  ff{ }}{ vv{ }}{  jj{ }}" format.name$ 't :=
      nameptr numnames = t "others" = and
        { ua.etal * }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "Der " #4
        "Die " #4
          "Das " #4
            "Ein " #4
              "Eine " #5
                  "The " #4 t chop.word
               chop.word
             chop.word
           chop.word
         chop.word
       chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.organization.sort}
{ author empty$
    { organization empty$
        { key empty$
            { "to sort, need author, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {editor.organization.sort.PWD}%% so war es in plainnat
{ editor empty$
    { organization empty$
        { key empty$
            { "to sort, need editor, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { editor sort.format.names }
  if$
}

FUNCTION {editor.organization.sort}%%das key-Feld soll z. Sortieren ben. werden
{ key empty$
    { editor empty$
       { organization empty$
            { "to sort, need editor, organization, or key in " cite$ * warning$
             ""
            }
            { "The " #4 organization chop.word sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { key sortify }
  if$
}

FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "booklet" =
  type$ "inbook" =
  or or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.organization.sort
        { type$ "manual" =
            'author.organization.sort
            'author.sort
          if$
        }
      if$
    }
  if$
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.label :=
  sort.label *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}

SORT

FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'longest.label.width :=
  #0 'last.extra.num :=
  #0 'number.label :=
}

FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}

FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
  label extra.label * 'label :=
  dinat.label extra.label * 'dinat.label :=
}

EXECUTE {initialize.longest.label}

ITERATE {forward.pass}

REVERSE {reverse.pass}

FUNCTION {bib.sort.order}
{ sort.label  'sort.key$ :=
}

ITERATE {bib.sort.order}

SORT

FUNCTION {begin.bib}
{   preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" *
  write$ newline$ newline$
  "% this bibliography is generated by nd24.bst [3.0c2] from 2005-12-21"
  write$ newline$ newline$
  "\providecommand{\natexlab}[1]{#1}"
  write$ newline$
  "\providecommand{\url}[1]{\texttt{#1}}"
  write$ newline$
  "\makeatletter"
  write$ newline$
  "\newcommand{\dinatlabel}[1]%"
  write$ newline$
  "{\ifNAT@numbers\else\NAT@biblabelnum{#1}\fi}"
  write$ newline$
  "\makeatother"
  write$ newline$
  "\expandafter\ifx\csname urlstyle\endcsname\relax"
  write$ newline$
  "  \providecommand{\doi}[1]{doi: #1}\else"
  write$ newline$
  "  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi"
  write$ newline$
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}
